Event-triggered Feedback Control for Signal Temporal Logic Tasks

A framework for the event-triggered control synthesis under signal temporal logic (STL) tasks is proposed. In our previous work, a continuous-time feedback control law was designed, using the prescribed performance control technique, to satisfy STL tasks. We replace this continuous-time feedback control law by an event-triggered controller. The event-triggering mechanism is based on a maximum triggering interval and on a norm bound on the difference between the value of the current state and the value of the state at the last triggering instance. Simulations of a multi-agent system quantitatively show the efficacy of using an event-triggered controller to reduce communication and computation efforts.

==> chapter/sequencing.tex <==
\section{Control strategy for sequential formulas}
\label{sec:sequencing}
In this section, we develop a hybrid control strategy for sequential formulas $\theta$ as in \eqref{eq:theta_class}, which either correspond to $\theta^{s_1}$ or $\theta^{s_2}$ as in \eqref{eq:theta1_class} or \eqref{eq:theta2_class}, respectively. Note that both of these consist of $N$ atomic temporal formulas: $\theta^{s_1}$ entails $N$ atomic temporal formulas $\phi_i$ with $[a_i,b_i]$ for all  $i\in\{1,\hdots,N\}$. Similarly, $\theta^{s_2}$ boils down to $N-1$ atomic temporal formulas $\phi_i=F_{[a_i,b_i]}\psi_i$ with $i\in\{1,\hdots,N-1\}$, $a_{i}:=\sum_{k=1}^ic_k$, $b_i:=\sum_{k=1}^id_k$,  and $\phi_N$. For instance, $F_{[c_1,d_1]}\big(\psi_1 \wedge F_{[c_2,d_2]}(\psi_2 \wedge F_{[c_3,d_3]}\psi_3)\big)$ is satisfied if and only if $F_{[c_1,d_1]}\psi_1 \wedge F_{[c_1+c_2,d_1+d_2]}\psi_2 \wedge  F_{[c_1+c_2+c_3,d_1+d_2+d_3]}\psi_3:=F_{[a_1,b_1]}\psi_1 \wedge F_{[a_2,b_2]}\psi_2 \wedge  F_{[a_3,b_3]}\psi_3$ is satisfied. To conclude, $\theta$ consists of $N$ atomic temporal formulas $\phi_i$ with $i\in\{1,\hdots,N\}$. Each $\phi_i$ entails a robustness function denoted by $\rsnt{\psi_i}$ and corresponding design parameters $t_{i,*}$, $r_i$, $\rho_{i,max}$, and $\gamma_i(t)=(\gamma_{i,0}-\gamma_{i,\infty})\exp(-l_{i}t)+\gamma_{i,\infty}$ in accordance with $t_*$, $r$, $\rho_{max}$, and $\gamma$ in Section \ref{sec:strategy}.  Each $\phi_i$ will be processed one at a time. If $\phi_i$ has been satisfied, the next atomic temporal formula $\phi_{i+1}$ becomes active and a switch takes place. Denote the time sequence of these switching times by $\{\Delta_1:=0,\Delta_2,\hdots,\Delta_N\}$ where $\Delta_i\le \Delta_{i+1}$. Note that $t_{i,*}$, $r_i$, $\rho_{i,max}$, $\gamma_{i,0}$, $\gamma_{i,\infty}$, and $l_i$ need to be calculated during runtime at each switching time $\Delta_i$. Furthermore, set $p:=\begin{cases} 1  \text{ if } \theta=\theta^{s_1}\\ 0 \text{ if } \theta=\theta^{s_2} \end{cases}$  and $m_i:=\begin{cases} 1 \text{ if } \phi_i=G_{[a_i,b_i]}\psi_i \\ 0  \text{ if } \phi_i=F_{[a_i,b_i]}\psi_i. \end{cases}$

A hybrid control strategy in the framework introduced in Definition \ref{def:hybrid_system} will be used to process each $\phi^i$ sequentially.
\begin{definition}\cite{goebel2012hybrid}\label{def:hybrid_system}
	A hybrid system is a tuple $\mathcal{H}:=(C,F,D,G)$, where $C$, $D$, $F$, and $G$ are the flow and jump set and the possibly set-valued flow and jump map, respectively. The discrete and continuous dynamics are 
	\begin{align*}
	\begin{cases}
	\dot{\boldsymbol{z}}\in F(\boldsymbol{z}) & \text{if }\boldsymbol{z} \in C  \\
	\boldsymbol{z}^+\in G(\boldsymbol{z}) & \text{if }\boldsymbol{z} \in D. 
	\end{cases}
	\end{align*}
\end{definition}


Define $\boldsymbol{p}_f:=\begin{bmatrix} t_* & r & \rho_{max} & \gamma_{0} & \gamma_{\infty} & l \end{bmatrix}^T$, gathering all parameters defining the funnel in \eqref{eq:inequality}, and the hybrid state $\boldsymbol{z}:=\begin{bmatrix} q & \boldsymbol{x}^T & t & \Delta & \boldsymbol{p}_f^T  \end{bmatrix}^T\in \{1,\hdots,N+1\}\times \mathbb{R}^n \times \mathbb{R}_{\ge 0}^8 =:\mathcal{Z}$. Note that $\Delta$ is the value of the latest switching time. In adherence to the terminology in \cite{goebel2012hybrid}, we interchangeably call switches jumps. The discrete state $q$ indicates which formula $\phi_q$ is currently active, while $q=N+1$ indicates the final discrete state when $\theta$ has already been satisfied. In the proof of Theorem \ref{theorem:3}, it was shown that $\boldsymbol{x}(t)\in\Omega_{\boldsymbol{x}}^\prime$ for all $t\in\mathbb{R}_{\ge 0}$, where $\Omega_{\boldsymbol{x}}^\prime$ is a compact set.  Let $\Omega_{q,\boldsymbol{x}}^\prime$ denote $\Omega_{\boldsymbol{x}}^\prime$ corresponding to the formula $\phi_q$. Next, define the sets $\mathcal{X}_q:=\{\boldsymbol{x}\in\mathbb{R}^n|r_q<\rsnt{\psi_q}<\rho_{q,max}\}$ and $\mathcal{Y}_q:= [0,{b_q}^p+{\big(\sum_{i=1}^qd_i\big)}^{1-p}-1] \times t_{q,*} \times r_q \times \rho_{q,max} \times \gamma_{q,0} \times \gamma_{q,\infty} \times l_{q}$. Note that $p$ determines if $[a_q,b_q]$ or $[c_q,d_q]$ is used. For all $q\in\{1,\hdots,N\}$, set
\begin{small}
	\begin{align}\label{eq:t_star}
	t_{q,*}\in
	\begin{cases}
	a_q &\text{if } p=1, m_q=1\\
	[a_q,b_q] &\text{if } p=1, m_q=0\\
	c_q &\text{if } p=0, m_q=1\\
	[c_q,d_q] &\text{if } p=0, m_q=0.\\
	\end{cases}
	\end{align} 
\end{small}
Next, define the set $\mathcal{D}_{q}$ that indicates satisfaction of $\phi_q$ and leads to a jump to process $\phi_{q+1}$. For $q\in\{1,\hdots,N\}$, define 
\begin{small}
	\begin{align*}
	\mathcal{D}_{q}:= \begin{cases}
	q \times \mathcal{X}_q \times ({b_q}^p+{d_q}^{1-p}-1-p\Delta)  \times \mathcal{Y}_q \hspace{0.69cm} \text{if } m_q=1\\ 
	q \times \mathcal{X}_q \times ([{a_q}^p+{c_q}^{1-p}-1,t_{q,*}]-p\Delta) \times  \mathcal{Y}_q \;\text{if } m_q=0,
	\end{cases}
	\end{align*} 
\end{small}which indicates that $\rsq{\phi_q}>r_q$ if $\boldsymbol{z}\in\mathcal{D}_{q}$. This follows since $\boldsymbol{x}\in\mathcal{X}_q$ at $t={b_q}^p+{d_q}^{1-p}-1-p\Delta$ for $m_q=1$ or $\boldsymbol{x}\in\mathcal{X}_q$ at $t\in ([{a_q}^p+{c_q}^{1-p}-1,t_{q,*}]-p\Delta)$ for $m_q=0$ under the control law \eqref{equ:control} indicates that $\phi_q$ is satisfied.  Note that $\Delta$ only takes effect if $p=1$ ($\theta=\theta^{s_1}$) to ensure that $\phi_q$ is satisfied within $[a_q,b_q]$, while for $p=0$ ($\theta=\theta^{s_2}$) the formula $\phi_{q+1}$ is directly processed next when $\phi_q$ is satisfied. Further define $\mathcal{D}_{N+1}:=(N+1) \times \Omega_{N,\boldsymbol{x}}^\prime \times T  \times \mathcal{Y}_N$ for $T:={b_N}^p+(\sum_{i=1}^Nd_i)^{1-p}-1$, which is needed for a technical reason in the proof of Theorem \ref{theorem:hybrid_system}. Similarly, define the continuous domain $\mathcal{C}_q$ for $q\in\{1,\hdots,N\}$ as 
\begin{small}
	\begin{align*}
	\mathcal{C}_{q}:=
	\begin{cases}
	q\times \Omega_{q,\boldsymbol{x}}^\prime \times [0, {b_q}^p+{d_q}^{1-p}-1-p\Delta] \times \mathcal{Y}_q \;\;\text{if } m_q=1\\
	q \times \text{cl}(\Omega_{q,\boldsymbol{x}}^\prime\setminus \mathcal{X}) \times [0, t_{q,*}-p\Delta] \times \mathcal{Y}_q \hspace{1.05cm}\text{if } m_q=0,
	\end{cases}
	\end{align*}
\end{small}where cl($\cdot$) denotes the closure. Also define $\mathcal{C}_{N+1}:=(N+1)\times \Omega_{N,\boldsymbol{x}}^\prime\times [0,T]  \times \mathcal{Y}_N$.  Finally, the jump and flow sets are given by   
\begin{align*}
D&:=  \cup_{i=1}^{N+1}  \mathcal{D}_{i}  \\
C&:= \cup_{i=1}^{N+1} \mathcal{C}_{i}.
\end{align*} 
The flow map is given by 
\begin{align*}
F:=\begin{bmatrix} 0 & {\big(f(\boldsymbol{x})+g(\boldsymbol{x})\boldsymbol{u}_q+\boldsymbol{w}\big)}^T & 1 & {\boldsymbol{0}_7}^T\end{bmatrix}^T
\end{align*} 
with the control law in \eqref{equ:control} as $\boldsymbol{u}_{q}=-\epsilon_q g^T(\boldsymbol{x}) \frac{\partial \rsnt{\psi_q}}{\partial \boldsymbol{x}}$ for all $q\in \{1,\hdots,N\}$ and $\boldsymbol{u}_{N+1}=-\epsilon_N g^T(\boldsymbol{x}) \frac{\partial \rsnt{\psi_N}}{\partial \boldsymbol{x}}$, where $\epsilon_q$  corresponds to $\epsilon$  based on $\phi_q$. By abbreviating $q^\prime:=q+1$, define $\boldsymbol{p}_s(q):=\begin{bmatrix}
q^\prime & \boldsymbol{x}^T & 0 & \Delta_{q^\prime} & t_{q^\prime,*} & r_{q^\prime} & \rho_{q^\prime,max} &\gamma_{q^\prime,0} & \gamma_{q^\prime,\infty} &l_{q^\prime} 
\end{bmatrix}^T$. Then, the jump map is given by
\begin{small}
	\begin{align*}
	G:=
	\begin{cases}
	{\boldsymbol{p}_s(q)} \hspace{3.22cm}
	\text{if}\; q\notin\{N,N+1\}, \boldsymbol{z}\in D \\ 
	\begin{bmatrix}
	N+1 & \boldsymbol{x}^T & \boldsymbol{0}_2^T & {\boldsymbol{p}_f}^T 
	\end{bmatrix}^T 
	\;\text{if}\; q\in\{N,N+1\}, \boldsymbol{z}\in D,  
	\end{cases}
	\end{align*}
\end{small}where we set $\Delta_{q^\prime}:=\Delta+t$, accumulating the elapsed time after jumps. Select $t_{q^\prime,*}$ as in \eqref{eq:t_star},  $\rho_{q^\prime,max}\in \big(\max(0,\rsnt{\psi_{q^\prime}}),\rso{\psi_{q^\prime}}\big)$, and $r_{q^\prime}\in[0,\rho_{q^\prime,max})$ as in the assumptions of Theorem \ref{theorem:3} and \ref{lemma:gamma}, respectively. The parameters $\gamma_{i,0}$, $\gamma_{i,\infty}$, and $l_i$ need to be chosen as in \eqref{eq:g1}, \eqref{eq:g2}, and \eqref{eq:g3}: $\gamma_{q^\prime,0}\in\begin{cases}(\rho_{q^\prime,max}-\rsnt{\psi_{q^\prime}},\infty)&\text{if } t_{q^\prime,*}-p\Delta_{q^\prime}>0\\ (\rho_{q^\prime,max}-\rsnt{\psi_{q^\prime}},\rho_{q^\prime,max}-r_{q^\prime}]&\text{if } t_{q^\prime,*}-p\Delta_{q^\prime}=0 \end{cases}$, $\gamma_{q^\prime,\infty}\in \Big(0,\min\big(\gamma_{q^\prime,0},\rho_{q^\prime,max}-r_{q^\prime}\big)\Big]$, and 
\begin{small}
\begin{align*}
l_{q^\prime}\in
\begin{cases}
\mathbb{R}_{\ge 0} \hspace{3.025cm} \text{if }  -\gamma_{q^\prime,0}+\rho_{q^\prime,max}\ge r_{q^\prime}\\
-\frac{\ln\big(\frac{r_{q^\prime}+\gamma_{q^\prime,\infty}-\rho_{q^\prime,max}}{-(\gamma_{q^\prime,0}-\gamma_{q^\prime,\infty})}\big)}{t_{q^\prime,*}-p\Delta_{q^\prime}} \;\;\; \text{if: }\bullet -\gamma_{q^\prime,0}+\rho_{q^\prime,max}< r_{q^\prime},\\ \hspace{4.06cm} \bullet \;t_{q^\prime,*}-p\Delta_{q^\prime}>0.
\end{cases}
\end{align*} 
\end{small}Note that $G$ is hence a set-valued map. The initial state is set to $\boldsymbol{z}_0:=\begin{bmatrix}
1 & {\boldsymbol{x}_0}^T & 0 & 0 & t_{1,*} & r_{1} & \rho_{1,max} &\gamma_{1,0} & \gamma_{1,\infty} & l_{1}
\end{bmatrix}^T$.  Now, we are ready to state the main result of this section.

\begin{theorem}\label{theorem:hybrid_system}
	
	Consider the system \eqref{system_noise} and a formula $\theta$ as in \eqref{eq:theta_class}. The hybrid system $\mathcal{H}=(C,F,D,G)$ results in $r:=\min(r_1,\hdots,r_N)<\rsoo{\theta}<\rho_{max}:=\min(\rho_{1,max},\hdots,\rho_{N,max})$, i.e., $(\boldsymbol{x},0)\models\theta$, if each $\phi_q$ in $\theta$ is feasible w.r.t. $r_q$, $\boldsymbol{x}(\Delta_q)$, and $t_{q,*}+|p-1|\Delta_q$.


\begin{proof} 
First, note that the third case in the proof of Theorem \ref{lemma:gamma} is again excluded by the assumption of feasibility w.r.t. $r_q$, $\boldsymbol{x}(\Delta_q)$, and $t_{q,*}+|p-1|\Delta_q$. To show that $\theta$ is satisfied, we need to show that eventually $\phi_N$ is satisfied. Therefore, we show that the compact set $\mathcal{A}=(N+1)\times \bigcup \limits_{i=1}^{N}\Omega_{i,\boldsymbol{x}}^\prime \times [0,T]^3 \times [0,\max_i r_i]  \times [0,\max_i \rho_{i,max}] \times [0,\max_i \gamma_{i,0}] \times [0,\max_i \gamma_{i,\infty}] \times [0,\max_i l_{i}]$ is asymptotically stable. A hybrid Lyapunov-function candidate is $V(\boldsymbol{z}):=\big(q-(N+1)\big)^2$, which is positive on $(C\cup D) \setminus \mathcal{A}$. During flows it is easy to see that $\dot{V}=0$, while during jumps $V(\boldsymbol{z}^+)-V(\boldsymbol{z})=\big(q+1-(N+1)\big)^2-\big(q-(N+1)\big)^2=\big(q-N\big)^2-\big(q-(N+1)\big)^2<0$ for $q\in\{1,\hdots,N\}$. According to the invariance principle in \cite[Theorem 23]{goebel2009hybrid}, we now need to show that no complete solution can stay in $V(\boldsymbol{z})=\mu>0$. This is true due to the following fact: for each state $q=\{1,\hdots,N\}$, the control law  $\boldsymbol{u}_{q}(t)=-\epsilon_q g^T(\boldsymbol{x}) \frac{\partial \rsnt{\psi_q}}{\partial \boldsymbol{x}}$ of Theorem \ref{theorem:3} is applied to the system. Furthermore, $r_{q}$ and $\rho_{q,max}$ are chosen as in Theorem \ref{theorem:3} and \ref{lemma:gamma}, while $\gamma_{q,0}$, $\gamma_{q,\infty}$, and $l_{q}$ are chosen accordingly. This guarantees that each $\phi_q$ is satisfied with $\rho^{\phi_q}(\boldsymbol{x},\Delta_q)> r_q$. Hence, $\phi_q$ will eventually be satisfied and lead to a jump due to the structure of the jump set $D$, which decreases $V(\boldsymbol{z})$. Note that $\Delta_{q}$ ensures that each formula $\phi_q$ in $\theta^{s_1}$ is satisfied within $[a_q,b_q]$, while each $\phi_q$ in $\theta^{s_2}$ is processed without the use of $\Delta_q$. Hence, note that each solution is complete and it can be concluded that $\mathcal{A}$ is asymptotically stable, which leads to the conclusion that $\theta$ is satisfied with $r:=min(r_1,\hdots,r_N)<\rs{\theta}<\rho_{max}:=\min(\rho_{1,max},\hdots,\rho_{N,max})$.
\end{proof}
\end{theorem}


